Model Merging: Foundations and Algorithms

Modern deep learning usually treats models as separate artifacts: trained independently, specialized for particular purposes, and replaced when improved versions appear. This thesis studies model merging as an alternative paradigm: combining independently trained neural networks directly in weight space, with little or no optimization and without requiring access to the original training data. The thesis considers two main regimes. In the single-task setting, where models share an objective but differ in initialization, we introduce C$^2$M$^3$, a cycle-consistent merging algorithm based on Frank-Wolfe optimization. C$^2$M$^3$ aligns multiple networks into a shared, reference-free parameter space, making weight averaging meaningful without privileging any individual model. In the multi-task setting, where models are fine-tuned for different downstream tasks from a common pretrained initialization, we first develop a theoretical account of task vectors as approximate gradients. This explains both the effectiveness and the limitations of task arithmetic. Building on this view, we show that task vectors inherit the low-rank structure of gradients and introduce Task Singular Vectors (TSV), a decomposition that enables compression and interference reduction through TSV-Merge. We then present MASS, an input-adaptive routing method that uses TSV geometry to select task-relevant subspaces at inference time. Finally, we introduce MERGE$^3$, an evolutionary merging framework that uses Item Response Theory to reduce evaluation costs by up to 50$\times$ while preserving solution quality. Together, these contributions provide theoretical and algorithmic foundations for model merging, supporting a paradigm in which learned capabilities can be composed, reused, and extended across models.

==> 3_single_task/1_cycle_consistent/5_Related_work/content.tex <==
%!TEX root = ../../../main.tex
\textbf{Mode Connectivity and model merging.}
Mode connectivity studies the weights defining local minima.~\citet{linear-mode-connectivity} studied linear mode connectivity of models that were trained for a few epochs from the same initialization and related it to the lottery ticket hypothesis. Without requiring the same initialization, \citet{Entezari2021-me} speculated that all models share a single basin after having solved for the neuron permutations. 
Model merging aims at aggregating different models into a single one to inherit their capacities without incurring the cost and burden of ensembling. In this regard, \citet{model-fusion} proposed an optimal-transport-based weight-matching procedure, while \texttt{Git Re-Basin}~\cite{git-rebasin} proposed three matching methods and the \texttt{MergeMany} procedure seen in \cref{subsec:merging-n-models}. Subsequently, \texttt{REPAIR}~\cite{repair} showed that a significant improvement in performance of the interpolated model may be obtained by renormalizing its activations rather than changing the matching algorithm. 
Unlike all these works, we consider merging $n$ models and propose a principled way to perform it with cycle-consistency guarantees. 

\textbf{Cycle consistency.}
Ensuring cycle consistency of pairwise maps is a recurring idea in the computer vision and pattern recognition literature. In the realm of deep learning, earlier studies addressing multi-graph matching achieved cycle consistency by synchronizing the predicted pairwise permutations post hoc~\cite{wang08,NEURIPS2020_e6384711}. The alternative approach using an object-to-universe matching framework, which we adopt here, inherently ensures cycle consistency by construction, as demonstrated in~\cite{Bernard_2019_ICCV,huang13,10.1007/978-3-540-74936-3_45}. To the best of our knowledge, none of the existing works tackles cycle-consistent alignment of neural models. We refer to \cref{app:extended-related-work} for a more detailed list of related works.

==> 4_multi_task/0_background/content.tex <==
%!TEX root = ../../main.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% MULTI-TASK MERGING FOUNDATIONS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Background on multi-task merging}
\label{sec:multitask-merging-background}

As introduced in \cref{sec:landscape}, this part focuses on merging models that have been fine-tuned on different downstream tasks from a shared pre-trained backbone.
The central question is: \emph{can the knowledge acquired by individually fine-tuned models be combined into a single multi-task model, without retraining?} The shared initialization makes these models far more compatible than those trained from different random seeds, but simply averaging their parameters introduces destructive interference that grows with the number of tasks. This section reviews the key ideas and methods that form the technical foundation for the contributions in the following chapters.

\subsection{Task arithmetic}
\label{sec:task-arithmetic}

Among multi-task merging methods, \emph{task arithmetic}~\citep{task-vectors} stands out for its effectiveness and simplicity. The central abstraction is the \emph{task vector}: given a pre-trained model with parameters $\theta_0$ and a fine-tuned copy $\theta_t^*$ specialized on task $t$, the task vector is defined as the displacement
\begin{equation}
    \tau_t = \theta_t^* - \theta_0.
\end{equation}
This displacement isolates the direction in weight space that encodes the knowledge acquired during fine-tuning. The key insight is that these vectors can be composed through elementary arithmetic to edit the model's behavior. Two primitive operations define the framework. \emph{Addition} constructs a multi-task checkpoint by summing task vectors from different tasks:
\begin{equation}
    \theta_{\text{merge}} = \theta_0 + \lambda \sum_{t=1}^{T} \tau_t, \label{eq:task-arithmetic}
\end{equation}
where $\lambda$ is a scaling coefficient chosen on validation. This yields a single model that inherits competencies from all constituent tasks at no additional inference cost. \emph{Negation} subtracts a task vector, $\theta_0 - \lambda \tau_t$, to suppress a specific behavior (e.g., reducing toxicity) while approximately preserving the model's remaining capabilities.

Empirically, \citet{task-vectors} demonstrated that negating task vectors can sharply reduce targeted capabilities while addition yields functional multi-task models. However, performance degrades as the number of merged tasks grows, since naive summation treats all parameters uniformly and does not explicitly manage conflicts between task vectors.

\subsection{Mitigating multi-task interference}
\label{sec:mitigating-interference}

While task arithmetic is simple and often effective, standard nonlinear fine-tuning inevitably introduces inter-task interference when task vectors are summed. A natural line of work tackles this interference through post-hoc interventions on precomputed task vectors, identifying and removing the parameter-level conflicts responsible for performance degradation.

\citet{ties} diagnosed two concrete failure modes of naive task arithmetic: \emph{redundant parameters}, whose small magnitudes contribute noise rather than signal under averaging, and \emph{sign conflicts}, where different task vectors push the same parameter in opposite directions, causing destructive cancellation. Their TIES-Merging framework (Trim, Elect Sign, Disjoint merge) addresses both issues through a three-step pipeline: (i)~\emph{trim} each task vector by retaining only the top-$k\%$ of parameters by absolute magnitude; (ii)~\emph{elect} a dominant sign per coordinate via a majority vote weighted by magnitude; and (iii)~\emph{disjoint merge} by averaging only those entries whose sign agrees with the elected sign, discarding conflicting updates. Empirically, up to 80\% of delta parameters could be trimmed without statistically significant performance loss, and enforcing sign consistency substantially improved multi-task coherence, with gains growing as more tasks are merged.

A complementary perspective on parameter redundancy was offered by \citet{yu2024language} with \textsc{DARE} (Drop And REscale). For models obtained via supervised fine-tuning (SFT), the delta parameters tend to be remarkably small in magnitude, implying that the vast majority of individual updates are individually dispensable. DARE exploits this by randomly dropping a fraction $p$ of delta parameters (routinely $p \in [0.9, 0.99]$) and rescaling the survivors by $1/(1-p)$ to preserve the expected activation magnitude. The extreme sparsification dramatically reduces the probability of two task vectors interfering at the same coordinate, and the sparsified vectors can then be combined using standard task arithmetic or TIES. An important caveat is that DARE relies on the SFT deltas being small; when fine-tuning amounts to substantial continued pre-training, even moderate dropping rates cause catastrophic performance collapse.

As the number of merged tasks scales, even interference-aware methods like TIES exhibit degradation. \citet{wang2024localizing} investigated whether task information is truly destroyed by merging or merely hidden by interference, finding support for the latter view. Their TALL-masks framework constructs per-task binary masks $m_t$ that approximate each single-task vector from the dense multi-task vector $\tau_{\text{MTL}} = \sum_t \tau_t$, using a closed-form criterion that identifies coordinates where a task's own contribution dominates over the aggregate of all other tasks. Analyzing the intersection patterns of these masks reveals three regimes: \emph{selfish} weights critical to one task but harmful to others, \emph{catastrophic} weights that no task considers critical, and \emph{general} weights selected by multiple tasks forming a consensus backbone. The resulting \emph{Consensus Merging} strategy retains only general weights, yielding substantial improvements.

An alternative perspective is offered by \citet{tammerging}, who formulate merging as finding a solution in the \emph{task parameter subspace} (the span of the individual task vectors) that simultaneously approximates all single-task models. This reduces the problem to solving a linear system, which the authors tackle with the conjugate gradient method, achieving strong results in both multi-task and intermediate-task merging.

\citet{daheim2024model} framed merging as minimizing the mismatch between the gradients of the individual models and those of the merged model, proposing an uncertainty-based scheme that is more robust to hyperparameter choices than standard task arithmetic.

These methods share a common principle: multi-task interference can be substantially reduced by identifying and removing the specific parameter coordinates responsible for conflicts, or by finding better combinations within the space spanned by the task vectors. \Cref{ch:tsv} presents an alternative view rooted in spectral properties of the layer-wise weight updates.

\subsection{Routing-based merging}
\label{sec:routing-based}

Rather than committing to a single static merge, routing-based methods~\citep{he2023merging, moerging, tang2024smile, twinmerging} make composition input-dependent: at inference time, a gating mechanism selects or weights task-specific components, in the spirit of Mixture-of-Experts models. This preserves specialization while still sharing most backbone parameters. Existing approaches span a broad design space. In LLMs, several methods train routers over LoRAs or adapters~\citep{jang2023exploring, chronopoulou2023adaptersoup, muqeeth2024learning}, or softly merge expert modules via learned weighted combinations~\citep{muqeethsoft, ostapenko2024towards}. \citet{muqeethsoft} proposed \textsc{SMEAR}, which replaces discrete expert routing with a single merged expert formed by a differentiable weighted average of parameters, enabling standard gradient-based training. \citet{ostapenko2024towards} extended the idea of adapter libraries by introducing model-based clustering to organize LoRAs by similarity and a zero-shot routing mechanism (\textsc{Arrow}) that selects relevant adapters for new inputs without retraining. These approaches can require additional supervision or optimization. Other methods target post-hoc composition from existing checkpoints: some still depend on modified fine-tuning pipelines (e.g., \texttt{Transformer}$^2$~\citep{sun2025transformer2}), whereas others are explicitly data- and training-free, routing low-rank task updates at the layer level while leaving the pre-trained backbone unchanged. \Cref{ch:mass} presents one such approach.

\subsection{Optimization-based model merging}
\label{sec:coeff-optimization}

A complementary line of work casts model merging as an explicit optimization problem, rather than relying on fixed interpolation rules such as uniform averaging. Instead of retraining weights, these methods directly optimize a merging objective using information available at the endpoints, either in parameter space or through low-dimensional combination rules.

A canonical example is Fisher-weighted merging~\citep{matena_merging_2022}, which adopts a Bayesian perspective on model combination. Each fine-tuned model is approximated by a Gaussian posterior obtained via a second-order (Laplace) expansion of the loss around its optimum, with the diagonal Fisher information acting as a precision matrix. Merging then amounts to maximizing the joint posterior, yielding a closed-form solution in which each parameter is set to a Fisher-weighted average across models. This induces a geometry-aware merge that preserves parameters deemed important for each task while allowing flexibility along directions of low curvature.

More recently, black-box optimization strategies have been proposed to directly search for high-performing merges. Evolutionary approaches~\citep{sakana} treat model merging as a fitness-driven process, using validation performance to guide exploration over merging strategies. While this enables highly flexible, non-differentiable search and can discover strong merges in challenging settings, it incurs substantial computational cost due to repeated model evaluations. In \cref{ch:merge3}, we show how this cost can be drastically reduced while preserving the benefits of adaptive, objective-driven merging.

\subsection{Understanding why task arithmetic works}
\label{sec:tangent-space}

The methods reviewed so far operate on task vectors to improve merging performance, but a deeper question remains: under what conditions does task arithmetic succeed in the first place?

\citet{ortiz2024task} formalized a sufficient condition: task arithmetic succeeds when the model satisfies a \emph{locality property}, meaning each task vector affects the model's output only on the data support of its own task and leaves outputs unchanged elsewhere. When this non-interference condition holds, task vectors can be summed without mutual corruption.

The authors identified \emph{weight disentanglement} as the core enabling mechanism: when approximately orthogonal directions in parameter space govern separate regions of function space. Crucially, this disentanglement is not present at random initialization; it is an emergent consequence of large-scale pre-training. Standard nonlinear fine-tuning, however, introduces curvature that warps these directions, causing task vectors to interfere when summed.

To amplify disentanglement, the authors proposed performing fine-tuning in the \emph{tangent space} of the pre-trained model, i.e., linearizing the network via a first-order Taylor expansion around $\theta_0$:
\begin{equation}
    f(x; \theta) \approx f(x; \theta_0) + \nabla_\theta f(x; \theta_0)^\top (\theta - \theta_0).
\end{equation}
This linearization ensures that the resulting task vectors remain strictly in a regime where superposition is benign. The theoretical justification is grounded in an eigenfunction localization property: if the Neural Tangent Kernel eigenfunctions associated with different tasks have non-overlapping supports, the corresponding weight updates are orthogonal and non-interfering.

In practice, linear fine-tuning of CLIP ViT models improved absolute accuracy on multi-task addition by up to 5 points and task negation by up to 13 points compared to standard nonlinear fine-tuning. While this confirms the centrality of disentanglement, the approach has a practical limitation: it requires modifying the fine-tuning procedure itself, and thus cannot be applied post-hoc to existing checkpoints.

In this regime, parameter updates are entirely determined by first-order loss gradients evaluated at $\theta_0$, with higher-order curvature effects explicitly suppressed. If linearization around $\theta_0$ is the regime where task arithmetic is most principled, then task vectors should be closely related to the accumulation of early training gradients evaluated near $\theta_0$. \Cref{ch:gradient} makes this connection precise, showing that task vectors from short fine-tuning are approximate negative gradients, and that this viewpoint yields both theoretical guarantees and practical improvements.

% \paragraph{Layer-wise perspective.}
% A finer-grained view considers these operations at the individual layer level. The per-layer \emph{task matrix} for task $i$ at layer $\ell$ is $\Delta_i^{(\ell)} = \theta_{\text{ft}_i}^{(\ell)} - \theta_0^{(\ell)}$, and the merged weights become $\theta_\text{MT}^{(\ell)} = \theta_0^{(\ell)} + \lambda \sum_{i=1}^T \Delta_i^{(\ell)}$. When the layer has a matrix structure, this preserves structural information that is lost when treating the full model as a flat vector. This layer-wise perspective is central to several chapters in this thesis.


==> 4_multi_task/1_task_vectors_gradients/1_Introduction/content.tex <==
%!TEX root = ../../../main.tex
Having addressed single-task merging in \cref{part:setting-one}, we now turn to the multi-task regime introduced in \cref{sec:multitask-merging-background}. The shared pre-trained backbone makes independently fine-tuned models far more compatible than those trained from different random seeds, eliminating the need for explicit alignment. Yet a new difficulty arises: when multiple task vectors are simply summed, they interfere with one another in ways that degrade per-task performance. Understanding this interference calls for a theoretical account of what task vectors actually encode.

As introduced in \cref{sec:task-arithmetic}, task arithmetic constructs a multi-task model by summing the task vectors of individually fine-tuned models.
\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{images/teaser.pdf}
    \caption[Task vectors as negative gradients under single-epoch GD]{Left: endpoint models are fine-tuned with SGD for more than one epoch. Right: endpoint models are fine-tuned with GD for a single epoch, making task vectors equivalent to negative gradients.}
    \label{fig:teaser}
\end{figure}
Despite its widespread adoption, a rigorous understanding of \emph{why} task arithmetic works has remained elusive. Prior work \citep{zhou2025atmimprovingmodelmerging, twinmerging, horoi2025less} has observed that task vectors from shorter fine-tuning, although less performant on the individual task, are better suited for merging, but without a formal explanation.

This chapter bridges the gap by connecting task vectors to gradient descent dynamics. Under full-batch GD, a task vector from one epoch of fine-tuning is precisely the negative loss gradient scaled by the learning rate (\cref{fig:teaser}). Summing these vectors therefore recovers a single GD step on the aggregated multi-task loss, with the scaling factor $\alpha$ acting as an effective learning rate. For multi-epoch fine-tuning the equivalence holds approximately, with an $O(\eta^2)$ deviation controlled by loss curvature.

These results carry a practical implication: merging models fine-tuned for a single epoch can match or exceed the performance of merging fully converged models, since first-epoch task vectors are the most faithful gradient approximations. More broadly, they reframe task arithmetic as approximate multi-task gradient descent and highlight the outsized role of early training dynamics.



==> 4_multi_task/1_task_vectors_gradients/5_Related_work/content.tex <==
%!TEX root = ../../../main.tex
\textbf{Mode Connectivity and Model Merging:}    Mode connectivity studies how weights characterize local minima. \citet{linear-mode-connectivity} showed linear paths exist between models with shared initialization, and \citet{Entezari2021-me} demonstrated convergence to a shared basin post-permutation. Permutation-based merging builds on this, with methods like optimal transport matching~\citep{model-fusion}, \texttt{Git Re-Basin}~\citep{git-rebasin}, and \texttt{REPAIR}~\citep{repair}. More recent approaches explore embedding-space merging~\citep{navon2023equivariant} and cycle-consistent alignment~(\cref{ch:cycle-consistent}). Averaging techniques beyond simple averaging~\citep{wortsman2022model}, such as population-based merging~\citep{jolicoeur2023population}, RegMean~\citep{jin2022dataless}, and Fisher-weighted merging~\citep{matena_merging_2022}, optimize merging coefficients in the weighted average. Post-merge performance has been shown to suffer from gradient mismatches between individual models~\citep{gradient-mismatch}. \citet{choshen2022fusing} introduced a method of merging fine-tuned models to produce an initialization superior to pre-training, leading to improved downstream performance when subsequently fine-tuned on a target task.

\textbf{Task Vectors:}   Task vector methods~\citep{task-vectors} represent task-specific updates as deltas from a shared model, enabling arithmetic operations for transfer, forgetting, and composition. Extensions reduce interference via sparsity~\citep{panda2024lottery}, pruning~\citep{yadavties, davari2025model}, masking~\citep{yu2024language}, and optimization~\citep{yangadamerging}. Some add test-time adaptation via learned modules~\citep{yang2024representation} or advocate disentangled fine-tuning in tangent space~\citep{ortiz2024task}. While these works enhance task vectors post-hoc, several works have explored how the duration of fine-tuning affects model merging. Specifically, \citet{zhou2025atmimprovingmodelmerging, twinmerging, horoi2025less}  highlighted the advantage of merging early task vectors that are fine-tuned for short intervals, yet exhibiting premature task-specific performance. To the best of our knowledge, our work provides the first rigorous theoretical foundation for this phenomenon.

%\paragraph{Federated Averaging}
%\AAAA is structurally similar to FedAvg~\citep{mcmahan2017communication}, alternating between local updates and aggregation from shared initialization. However, unlike FedAvg's focus on privacy and data heterogeneity, \AAAA targets model merging, bridging federated learning and multi-task adaptation.

\textbf{Multi-Task Learning:} Multi-task learning (MTL) is a learning paradigm that aims to improve the generalization performance of multiple related tasks by learning them jointly. Early foundational work \citep{10.1023/A:1007379606734} established that MTL can enhance performance by leveraging shared representations and inductive biases across tasks. Subsequent studies \citep{zamir2018taskonomy} have demonstrated that identifying and exploiting the structure among visual tasks can lead to significant reductions in labeled data requirements while maintaining performance. However, MTL presents optimization challenges, particularly due to gradient interference between tasks. Methods like Gradient Surgery \citep{yu2020gradient} address this by orthogonally projecting gradients to mitigate conflicts. Similarly, \citet{liu2021conflict} introduces strategies to balance objectives and ensure convergence. Our theory and experiments show task vectors closely align with task gradients, especially in single-epoch fine-tuning, suggesting that merging such models can effectively approximate multi-task learning.


%MTL improves generalization by jointly learning shared representations~\citep{10.1023/A:1007379606734, zamir2018taskonomy}. It also poses challenges like gradient interference, addressed by gradient surgery~\citep{yu2020gradient} and task balancing~\citep{liu2021conflict}. We reinterpret model merging as approximating multi-task gradient descent. Our theory and experiments show task vectors closely align with task gradients, especially in single-epoch fine-tuning, suggesting that merging such models can effectively approximate multi-task learning.

%Our analysis centers around a similar high-level goal with MTL, as task arithmetic also seeks to effectively handle multiple tasks with a single model. However, while traditional MTL approaches typically involve joint training of all tasks, task arithmetic achieves this by merging individually trained models. \citet{wei2025modeling} frames model merging as a constrained optimization problem, projecting gradients onto a shared space of all tasks. 

==> 4_multi_task/1_task_vectors_gradients/6_Conclusions/content.tex <==
%!TEX root = ../../../main.tex
This chapter established a formal connection between task vectors and loss gradients. After a single epoch of gradient descent, a task vector is exactly the scaled negative gradient; applying task arithmetic is therefore equivalent to one step of joint multi-task training. For multi-epoch fine-tuning the equivalence holds approximately, with a quantifiable $O(\eta^2)$ error bounded explicitly for feed-forward networks. Empirical investigation across multiple vision benchmarks corroborates this picture: the first-epoch gradient dominates the fine-tuning trajectory in both magnitude and direction, and merging single-epoch models matches the performance of merging fully converged ones.

The gradient interpretation also carries a structural implication. If a task vector approximates the negative gradient of the task loss, it encodes a specific \emph{direction} in weight space pointing toward lower loss for that task. Does this directional information have further exploitable structure? In \cref{ch:tsv}, we answer affirmatively, showing that per-layer task matrices are intrinsically low-rank and leveraging this structure to simultaneously compress task vectors and reduce inter-task interference.

==> 4_multi_task/1_task_vectors_gradients/TA_and_MTL/content.tex <==
%!TEX root = ../../../main.tex
% ARCHIVED: This section discussed connections to iterative task arithmetic (Zhou et al. 2025)
% and related experimental evidence. It is not included in the final thesis to keep the
% chapter focused on the formal theoretical contribution; the content may be useful for
% a future extended related-work chapter.
%
% Having formalized the relationship between task vectors and task gradients, and bounded their divergence, we now discuss how this relationship manifests in empirical multi-task performance.
% Our theoretical analysis suggests that task vectors obtained from shorter intervals of finetuning more closely resemble multi-task gradients, making them better suited for model merging. In other words, task arithmetic applied to such ``premature'' task vectors can more effectively simulate the dynamics of multi-task learning.

% Interestingly, prior work by \citet{zhou2025atmimprovingmodelmerging} provides experimental evidence consistent with this perspective. In their iterative framework, referred to here as \textbf{iterative task arithmetic}, they start from a pretrained base model, finetune each task for a short interval to obtain task vectors, merge these vectors via task arithmetic to produce a new base model, and repeat this process over multiple rounds. Their results show that, under a fixed total finetuning budget, increasing the merge frequency (and thus decreasing the finetuning interval per round) consistently improves multi-task performance. This aligns with our claim that early-stage task vectors are more aligned with multi-task gradients and therefore yield better merged models.

% \begin{figure}[h]
% \centering
% \begin{minipage}[t]{0.45\textwidth}
% \centering
% \includegraphics[width=\linewidth]{images/budget distributions.png}
% \caption{Effect of merge frequency under fixed finetuning budget (adapted from \citealp{zhou2025atmimprovingmodelmerging}).}
% \label{fig:ITA performance for budgets}
% \end{minipage}
% \hfill
% \begin{minipage}[t]{0.43\textwidth}
% \centering
% \includegraphics[width=\linewidth]{images/decreasingAccs.pdf}
% \caption{Multi-task performance across varying total budgets (adapted from \citealp{zhou2025atmimprovingmodelmerging}).}
% \label{fig:MTL performance for budgets}
% \end{minipage}
% \end{figure}

%\subsection{Fixed-Budget Merging with Varying Granularity}
%In the experiments of \citet{zhou2025atmimprovingmodelmerging}, the authors vary the merge frequency under a fixed total budget (e.g., $10$ epochs in total) by performing merging every $10$, $5$, $2$, or $1$ epochs. Each iteration starts from the most recent merged model rather than the original pretrained model. Despite the varying number of merges, the total compute remains constant.
% Although this setup is reminiscent of federated learning methods such as FedAvg~\citep{mcmahan2017communication}, the key difference is the use of task vector addition instead of weight averaging, and the focus on merging for improved multi-task generalization. Their findings show that more frequent merges, corresponding to shorter finetuning intervals, lead to higher multi-task performance, supporting our theoretical prediction.

% \subsection{Comparison Across Budgets}
% They further compare different merging strategies across total budgets, again showing that iterative task arithmetic continues to yield performance gains even at larger budgets, whereas other task arithmetic-based methods plateau. This reinforces our perspective that the beneficial properties of early-stage task vectors, namely their closer alignment with multi-task gradients, are a key factor in successful model merging.

==> 4_multi_task/2_task_singular_vectors/1_Introduction/content.tex <==
%!TEX root = ../../../main.tex
%
% Broader intro / context

The gradient perspective established in \cref{ch:gradient} reveals that task vectors encode structured, directional information about each task's loss landscape, information that a flat-vector treatment discards. Indeed, most multi-task merging methods treat entire networks as high-dimensional vectors, overlooking the layer-wise matrix structure of weight updates \citep{ties, yu2024language, jin2022dataless, rame_diverse_2023, matena_merging_2022, daheim2024model, davari2025model}. This flattened view limits these approaches to coarse-grained measures like cosine similarity for assessing inter-task interactions.

% Intro to our work
The approach developed here instead preserves the natural matrix structure of neural network layers.
The starting point is to examine per-layer task \emph{matrices}, which represent weight changes for each task, through singular value decomposition (SVD). This decomposition yields singular vectors and singular values that capture the most significant directions of variation within each layer. We term these singular vectors \emph{Task Singular Vectors} (TSVs), as they provide an interpretable basis for assessing task-specific contributions at each layer.
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/main_results_2.pdf}
    \caption[\method{TSV-M} merging accuracy on \model{ViT-L-14}]{Mean accuracy of a \model{ViT-L-14} merged over 8, 14, and 20 tasks respectively. By significantly surpassing existing methods, \method{TSV-M} establishes the new state of the art in model merging.}
    \label{fig:main-results}
\end{figure}
%
% Layer task matrices are low-rank
%
Since task vectors approximate gradients, they may inherit a well-documented property of gradients: low-rank structure. Gradients in deep networks have been repeatedly observed to be low-rank \citep{zhaogalore, sonthalia2025low}, and the effectiveness of LoRA \citep{hulora}, which reparametrizes weight updates as low-rank products, further supports this. Our analysis confirms that task matrices are indeed low-rank: only a small fraction of TSVs suffices to represent each layer's function with high fidelity.

% TSV-Compress
%
Building on this insight, we introduce \method{TSV-Compress} (\method{TSV-C}), a simple yet effective procedure to compress task vectors by a factor proportional to the number of tasks while maintaining $99\%$ of the original accuracy. Focusing on only a fraction of the most relevant TSVs for each task, \method{TSV-Compress} enables efficient storage and processing of task-specific information without sacrificing performance.

%
% Task interference measure
%
Beyond compression, examining how TSVs from different tasks align or diverge within each layer provides a fine-grained, geometrically grounded view of task interference, going beyond global similarity metrics like cosine similarity.
%
%
% Model merging
%
Building on this, we introduce \method{TSV-Merge} (\method{TSV-M}), which combines compression and interference reduction: it discards the least relevant singular vectors per task and then decorrelates the remaining ones via a whitening transformation. Across several benchmarks, \method{TSV-M} outperforms existing methods by an average of $\sim\!15$ percentage points.
All code is publicly available\footnote{\href{https://github.com/AntoAndGar/task_singular_vectors}{https://github.com/AntoAndGar/task\_singular\_vectors}}.


==> 4_multi_task/2_task_singular_vectors/2_Related_work/content.tex <==
%!TEX root = ../../../main.tex
\begin{table}[htbp]
    \centering
    \small
    \caption{Model merging approaches and their requirements.}
    \label{tab:prerequisites}
    \begin{tabularx}{\linewidth}{@{}ccccc@{}}
        \toprule
        \multirow{2}{*}{\textbf{Method}} & \textbf{Additional} & \textbf{Extra} & \multicolumn{2}{c}{\textbf{Validat. data}} \\
        & \textbf{training} & \textbf{storage} & \textbf{inputs} & \textbf{labels} \\ 
        \midrule
        Weight Avg. \cite{wortsman_model_2022} & \negxmark & \negxmark & \negxmark & \negxmark \\
        \midrule
        Fisher-Merg. \cite{matena_merging_2022} & \negxmark & \negxmark & \poscheckmark & \negxmark \\
        RegMean \cite{jin2022dataless} & \negxmark & \negxmark & \poscheckmark & \negxmark \\
        \midrule
        EMR-Merging \cite{huang2024emrmerging} & \negxmark & \poscheckmark & \negxmark & \negxmark \\
        TALL-Mask \cite{wang2024localizing} & \negxmark & \poscheckmark & \negxmark & \negxmark \\
        \rowcolor{gray!15} \textbf{TSV-C (Ours)} & \negxmark & \poscheckmark & \negxmark & \negxmark \\
        \midrule
        Task Arith. \cite{task-vectors} & \negxmark & \negxmark & \poscheckmark & \poscheckmark \\
        Ties-Merging \cite{ties} & \negxmark & \negxmark & \poscheckmark & \poscheckmark \\
        AdaMerging \cite{yang2023adamerging} & \poscheckmark & \negxmark & \poscheckmark & \negxmark \\
        Consensus-TA \cite{wang2024localizing} & \negxmark & \negxmark & \poscheckmark & \poscheckmark \\
        \rowcolor{gray!15} \textbf{TSV-M (Ours)} & \negxmark & \negxmark & \negxmark & \negxmark \\
        \bottomrule
    \end{tabularx}
\end{table}



\paragraph{Model Merging} offers an efficient alternative to ensembling by combining existing models without the need for further training. Several approaches address this by determining the neuron permutations that align the models into a shared optimization basin, after which the models are combined using a straightforward averaging method \citep{git-rebasin, repair, zip-it, rebasin-implicit-sinkhorn}; see also \cref{ch:cycle-consistent}. An alternative line of approaches focuses on the multi-task scenario, where a single pre-trained model is fine-tuned for different tasks \citep{task-vectors, ties, yu2024language, matena_merging_2022, wortsman_model_2022, davari2025model, wang2024localizing, zhou2025atmimprovingmodelmerging,shen2024efficient}. The prerequisites for methods in this category are outlined in \Cref{tab:prerequisites}.
%
\baseline{Task Arithmetic} \citep{task-vectors} introduces the concept of \emph{task vectors}, which are the weight differences between fine-tuned models and the pre-trained base model. By averaging these vectors, a merged multi-task model can be created; conversely, negating a task vector allows for forgetting a specific task.
%
\baseline{TIES} \citep{ties} addresses redundancies in model parameters by first selecting the top-$k$ most significant parameter changes and then constructing a sign vector based on the majority sign across all models. The latter is used to merge the task vectors disjointly, meaning the average is not computed when a parameter is zero or when parameters disagree in sign.
%
Similarly, \baseline{DARE} \citep{yu2024language} randomly resets redundant parameters to their pre-trained values and rescales the remaining parameters by a factor proportional to the dropped ones, aiming to reduce interference among tasks.
%
\baseline{Fisher Merging} \citep{matena_merging_2022} and \baseline{RegMean} \citep{jin2022dataless} merge models by performing weighted averaging, utilizing the Fisher information matrix and the inner product of input vectors, respectively.
% 
% 
\baseline{Model Breadcrumbs} \citep{davari2025model} focuses on merging only significant weights by discarding outliers and both minor and large perturbations in the fine-tuned parameters.
%
More recently, \citet{wang2024localizing} observed that tasks often utilize non-overlapping sets of weights. They propose two methods: the first, \baseline{TALL-Mask}, uses binary masks to activate important task-specific weights, requiring extra storage (as does our method \method{TSV-C}) for the masks. The second, \baseline{Consensus Merging}, leverages these masks to remove parameters that are important to less than two tasks.
Like our approach, \baseline{TwinMerging} \cite{twinmerging} and \baseline{SMILE} \cite{tang2024smile} apply SVD to layer task matrices. However, neglecting singular vector interference, they require a router to selectively activate a subset during inference.

Unlike existing approaches, our methods explicitly address task interference by decorrelating the singular vectors of different tasks, rather than averaging or selectively merging parameters. The compression step further isolates each task's most relevant components, storing only the essential singular directions.



\paragraph{SVD for Model Compression} A significant body of work explores low-rank decompositions for fully-connected and convolutional layers \citep{denil2013predicting, denton2014exploiting, jaderberg2014speeding, kolda2009tensor, garipov2016ultimate}, as well as tensor decompositions \citep{denton2014exploiting, kim2016compression, garipov2016ultimate}. These approaches typically achieve a layer-by-layer factorization of a trained network, focusing on minimizing the difference between the original and the low-rank approximated weight matrices. This is accomplished using techniques like SVD \citep{denton2014exploiting, garipov2016ultimate, jaderberg2014speeding, kolda2009tensor} or iterative optimization \citep{jaderberg2014speeding, kim2016compression}. While other methods such as weight quantization, knowledge distillation, and pruning exist, we utilize SVD not only for low-rank approximation and compression but also because its matrix decomposition properties make it particularly effective in analyzing and mitigating interference.


==> 4_multi_task/2_task_singular_vectors/3_Approach/content.tex <==
%!TEX root = ../../../main.tex
We now show how TSVs can be used for both compression and interference reduction.

\begin{figure}
  \centering
  \includegraphics[width=\linewidth]{figures/ViT-B-32_radar_combined.pdf}
  \caption[\model{ViT-B-32} merging accuracy across task sets]{Absolute accuracy of a \model{ViT-B-32} merged over 8, 14, and 20 tasks, respectively.}
  \label{fig:radar_chart}
\end{figure}

\subsection{TSV for compression}\label{subsec:tsv-compress}
%
When the task is known or inferred (e.g., via a router, as in Mixture-of-Experts~\cite{eigen2014learningfactoredrepresentationsdeep, shazeer2017} architectures), we can leverage the low-rank structure of per-layer task matrices (\cref{subsec:low-rank}) to compress them, retaining only the singular vectors of the relevant task. In \cref{ch:mass}, we show how the TSV subspaces themselves can serve as the basis for such a router, enabling task inference at test time without any additional training.
In particular, given a known or inferred task index $h$, we set other task components to zero, reducing \cref{eq:sum-of-rank-1-matrices-multi-task} to:
%
\begin{equation}
    \hat M = \sum_{i=1}^\ntasks \underset{[i=h]}{\mathds{1}} \sum_{j=1}^{k} \sigma_j^{i} u_j^{i} v_j^{i\top} = \sum_{j=1}^{k} \sigma_j^{h} u_j^{h} v_j^{h\top} = \hat{\Delta}_{h} \,.
\end{equation}
%
Only the top $k$ singular components of $\Delta_h$ are retained. We use the same $k$ for every task, chosen so that each layer is compressed by a factor of $\frac{1}{T}$ relative to the original dimension. Increasing $k$ improves the approximation but reduces the compression ratio.

\subsection{TSV for model merging} \label{subsec:tsv-merge}
When task identity is unknown, we aim to produce a single merged model that performs well across all tasks. To reduce singular task interference, we decorrelate the TSVs of different tasks by whitening the concatenated matrices $\hat{U}$ and $\hat{V}$, applying the transformation $X \mapsto X(X^\top X)^{-\frac{1}{2}}$.
%
For numerical stability, we reformulate whitening as an orthogonal Procrustes problem, seeking the orthogonal matrix $\hat{U}_\bot$ that minimizes the projection error:
%
\begin{equation}
    \min_{\hat{U}_\bot} \| \hat{U}_\bot - \hat{U} \|_F \quad \text{s.t.}~\hat{U}_\bot^\top \hat{U}_\bot = I \,,
\end{equation}
% 
and similarly for $\hat{V}$. This problem admits a closed-form solution via the SVD $\hat{U}=PDQ^\top$, yielding $\hat{U}_\bot = P Q^\top$ (similarly for $\hat{V}_\bot$).
%
\begin{proposition} \label{prop:whitening-procrustes}
    The transformations $X \mapsto  X(X^\top X)^{-\frac{1}{2}}$ (whitening) and $X \mapsto PQ^\top$ (Procrustes), where $X = PDQ^\top$ is the SVD of $X$, are equivalent.
\end{proposition}
\begin{proof}
    Given $X=PDQ^\top$ and recalling that $D^\top D=D^2$ for diagonal matrices, simple algebraic manipulation yields $X^\top X = Q D^2 Q^\top$. It follows that $(X^\top X)^{-1/2}=Q D^{-1} Q^\top$, therefore the whitening transformation can be rewritten as $X (X^\top X)^{-1/2}=(PDQ^\top)(Q D^{-1} Q^\top)=PDID^{-1}Q^\top=PQ^\top$, completing the proof.
\end{proof}
%
Once the (rank-reduced) TSV matrices $\hat{U}$ and $\hat{V}$ are decorrelated, we reconstruct the merged layer as in \cref{eq:sum-of-rank-1-matrices-multi-task}; see \cref{alg:tsvmerge} for the complete steps.

\begin{algorithm}
    \caption{\method{TSV-Merge}.}\label{alg:tsvmerge}
    \begin{algorithmic}[1]
        \REQUIRE Task matrices $\Delta_1, \dots, \Delta_T$, scaling factor $\alpha$
        \ENSURE Merged model weights $\theta_{\text{MT}}$
        \FOR{$i = 1$ to $T$} 
            \STATE Compute SVD: $\Delta_i = U_i \Sigma_i V_i^\top$
            \STATE Retain first $\frac{1}{T}$ singular components of $U_i$, $\Sigma_i$, and $V_i$
        \ENDFOR
        \STATE \textbf{Concatenate} the matrices:
        \STATE \quad $U \gets [U_1\,|\,U_2\,|\,\dots\,|\,U_T]$
        \STATE \quad $\Sigma \gets \text{block-diag}(\Sigma_1, \Sigma_2, \dots, \Sigma_T)$
        \STATE \quad $V \gets [V_1\,|\,V_2\,|\,\dots\,|\,V_T]$
        \STATE \textbf{Compute} the SVD of $U$ and $V$:
        \STATE \quad $U = P_U D_U Q_U^\top$ \qquad $V = P_V D_V Q_V^\top$
        \STATE \textbf{Obtain} the orthogonal matrices:
        \STATE \quad $U_\bot = P_U Q_U^\top$ \qquad $V_\bot = P_V Q_V^\top$
        \STATE \textbf{Reconstruct} the merged matrix:
        \STATE \quad $\hat{M} \gets U_\bot \Sigma V_\bot^\top$
        \STATE \textbf{Construct} merged model weights:
        \STATE \quad $\theta_{\text{MT}} \gets \theta_{\text{pre}} + \alpha \hat{M}$
        \STATE \textbf{return} $\theta_{\text{MT}}$
    \end{algorithmic}
\end{algorithm}

==> 4_multi_task/2_task_singular_vectors/6_Conclusions/content.tex <==
%!TEX root = ../../../main.tex
This chapter showed that per-layer task matrices are inherently low-rank and introduced a geometrically grounded measure of task interference based on the alignment of singular vectors across tasks.

These insights yield two practical tools. \method{TSV-Compress} reduces task vectors by a factor of $\ntasks$ while retaining 99\% of accuracy, with constant storage independent of the number of tasks. \method{TSV-Merge} combines low-rank approximation with Procrustes-based interference reduction, achieving up to 97\% normalized accuracy. The ablation study reveals a superadditive synergy between the two steps: compression makes interference reduction effective by reducing the dimensionality of the Procrustes problem.

% FUTURE WORK
Exploring alternative methods for task importance and rank approximation could be a valuable direction for future work. Currently, we use a uniform rank across tasks, approximating each task vector to \(\frac{1}{\ntasks}\) of the layer's dimensionality. However, techniques like those from \citet{idelbayev2020low} or optimal hard thresholds from \citet{6846297} could be applied to select the optimal rank for each task individually.

The low-rank structure of task matrices, established in this chapter, also opens a new question beyond static merging: if each task occupies a distinct low-dimensional subspace of the weight space, can we exploit this geometry at \emph{inference time}? All the methods studied so far produce a single, fixed merged model that is applied identically regardless of the input, a limitation that leaves per-task accuracy on the table. In \cref{ch:mass}, we relax this constraint and explore an input-adaptive paradigm: rather than committing to one static combination of task subspaces, the model routes each input to the most relevant task singular vectors at inference time.

\FloatBarrier



==> 4_multi_task/3_mass/preamble.tex <==
%!TEX root = ../../main.tex
\usepackage{etoolbox}
\newtoggle{arxiv}
\toggletrue{arxiv} % or \togglefalse{arxiv}


\usepackage{amsthm}
\usepackage{amsmath}
\usepackage{multirow}
\usepackage{scalerel}
\usepackage{placeins}
\usepackage{url}
\usepackage{booktabs}
\usepackage{amsmath, amsfonts}
\usepackage{overpic}
\usepackage{amssymb}
\usepackage{appendix}
\usepackage{todonotes}
\usepackage{leftindex}
\usepackage{caption}
% \usepackage[linesnumbered, vlined]{algorithm2e}
\usepackage{algorithm}
\usepackage{algorithmic}
\usepackage{xcolor}
\usepackage[inline]{enumitem}
%\usepackage{algcompatible}
\usepackage{subcaption}

\usepackage{tikz}
\usetikzlibrary{3d}  % optional, for easier 3D transforms
\usepackage{tikz-3dplot}
\usepackage{algorithmic}
\usepackage{dsfont}
\usepackage{colortbl}
\usepackage{tabularx}

\usepackage{wrapfig}
\usepackage{arydshln}
\usepackage[most]{tcolorbox} 

\newcommand{\ntasks}{T}
\newcommand{\fix}{\marginpar{FIX}}
\newcommand{\new}{\marginpar{NEW}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% METHODS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\approach}[0]{\texttt{MASS}}
\newcommand{\oracle}[0]{\texttt{oracle-MASS}}
\newcommand{\batched}[0]{\texttt{batched-MASS}}
\newcommand{\nn}[0]{\texttt{nn-MASS}}
\newcommand{\linear}[0]{\texttt{linear-MASS}}
\newcommand{\proj}[0]{\texttt{proj-MASS}}

% \newcommand{\oracle}[0]{\oracletag-\texttt{MASS}}
% \newcommand{\nn}[0]{\nntag-\texttt{MASS}}
% \newcommand{\linear}[0]{\lintag-\texttt{MASS}}
% \newcommand{\proj}[0]{\projtag-\texttt{MASS}}


% Define the methodtag macro
\newcommand{\methodtag}[2]{%
  \tikz[baseline=(char.base)]{%
    \node[
      fill=#1,
      rounded corners=2pt,
      text=white,
      font=\bfseries,
      % Force the node to be a fixed size
      minimum width=1em,
      minimum height=1em,
      % Keep text centered in the forced-size box
      align=center,
      inner sep=0pt
    ](char){#2};%
  }%
}


% \newcommand{\nntag}{\protect\methodtag{mygreen}{N}}
% \newcommand{\lintag}{\protect\methodtag{mygreen}{L}}
% \newcommand{\projtag}{\protect\methodtag{mygreen}{P}}
% \newcommand{\oracletag}{\protect\methodtag{mygreen}{O}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% THEOREMS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{assumption}[theorem]{Assumption}
\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}


\definecolor{mygreen}{RGB}{129, 178, 154}
\definecolor{myblue}{RGB}{51, 92, 103}
\definecolor{myyellow}{RGB}{224, 159, 62}
\definecolor{myred}{RGB}{158, 42, 43}
\definecolor{mydarkred}{RGB}{84, 11, 14}
\definecolor{mywhite}{RGB}{255, 243, 176}
\definecolor{firebrick}{RGB}{178, 34, 34}

\newcommand{\dataset}[1]{\texttt{#1}}
\newcommand{\model}[1]{\texttt{#1}}

\newcommand{\method}[1]{\texttt{#1}}
\newcommand{\baseline}[1]{\texttt{#1}}

\newcommand{\vitsmall}[0]{\model{ViT-B-32}}
\newcommand{\vitmedium}[0]{\model{ViT-B-16}}
\newcommand{\vitlarge}[0]{\model{ViT-L-14}}

\newcommand{\negxmark}{\large\color{firebrick}{×}}
\newcommand{\poscheckmark}{\large\color{mygreen}{\checkmark}}

\newcommand{\improv}[1]{\textcolor{mygreen}{(+#1)}}
\newcommand{\worse}[1]{\textcolor{firebrick}{(-#1)}}

\newcommand{\posxmark}{\color{mygreen}{×}}
\newcommand{\negcheckmark}{\color{firebrick}{\checkmark}}

\newcommand{\act}{\mathbf{z}_{\ell}}


% It is strongly recommended to use hyperref, especially for the review version.
% hyperref with option pagebackref eases the reviewers' job.
% Please disable hyperref *only* if you encounter grave issues, 
% e.g. with the file validation for the camera-ready version.
%
% If you comment hyperref and then uncomment it, you should delete *.aux before re-running LaTeX.
% (Or just hit 'q' on the first LaTeX run, let it finish, and you should be clear).
\definecolor{iccvblue}{rgb}{0.21,0.49,0.74}
\usepackage[pagebackref,breaklinks,colorlinks,allcolors=iccvblue]{hyperref}
\usepackage[capitalize]{cleveref} %added this because ref to Proposition shows Theorem instead

% CRULE DASH LINE
\makeatletter
\def\adl@drawiv#1#2#3{%
        \hskip.5\tabcolsep
        \xleaders#3{#2.5\@tempdimb #1{1}#2.5\@tempdimb}%
                #2\z@ plus1fil minus1fil\relax
        \hskip.5\tabcolsep}
\newcommand{\cdashlinelr}[1]{%
  \noalign{\vskip\aboverulesep
           \global\let\@dashdrawstore\adl@draw
           \global\let\adl@draw\adl@drawiv}
  \cdashline{#1}
  \noalign{\global\let\adl@draw\@dashdrawstore
           \vskip\belowrulesep}}
\makeatother


\newcommand{\vertical}[1]{\rotatebox[origin=c]{90}{#1}}
\newcommand{\Comment}[1]{\hfill \textcolor{gray}{\# #1}}



\newcommand{\methodimagetag}[1]{%
  % 1. #1 = fill color
  % 2. #2 = file name (without .ext if you like)
  % 3. #3 = text that follows (optional)
  \tikz[baseline=(char.base)]{%
    \node[
      anchor=base, % <--- ensures the node baseline aligns with text baseline
      fill=white,
      rounded corners=1pt,
      % If you don't want text color, remove the next line.
      text=white,
      font=\bfseries,
      minimum width=1em,
      minimum height=1em,
      align=center,
      inner sep=0pt
    ](char){\includegraphics[height=0.9em]{#1}};%
  }%
}

\DeclareMathOperator*{\argmax}{arg\,max}



% TO HAVE A SEPARATE ToC FOR THE APPENDIX
% Define a custom table of contents for the appendix
\newcommand{\listofappendices}{%
    \begingroup
    \cftsetindents{section}{0em}{2.5em} % Adjust the indent as needed
    \renewcommand{\cftsecfont}{\bfseries}
    \renewcommand{\cftsecpagefont}{\bfseries}
    \tableofcontents
    \endgroup
}





==> 4_multi_task/3_mass/sec/2_background.tex <==
%!TEX root = ../../../main.tex
\paragraph{Notation}\label{subsec:mass-background}
%
We adopt the task arithmetic and layer-wise notation of \cref{sec:task-vectors-background}: $\Delta_i^{(\ell)} = \theta_{\text{ft}_i}^{(\ell)} - \theta_\text{pre}^{(\ell)}$ is the per-layer task matrix, and merging sums these updates as $\theta_\text{MT}^{(\ell)} = \theta_\text{pre}^{(\ell)} + \alpha \sum_{i=1}^\ntasks \Delta_i^{(\ell)}$. The layer index is omitted when clear from context. Each task matrix admits an SVD $\Delta_i = U_i \Sigma_i V_i^\top$; the \method{TSV-M} procedure of \cref{ch:tsv} retains the top-$k$ singular components and orthogonalizes them across tasks to reduce interference. The full merging step is detailed in \cref{alg:fixed-merging} (lines \ref{line:start-fixed_merging}--\ref{line:end-fixed_merging}).

==> 4_multi_task/3_mass/sec/5_discussion.tex <==
%!TEX root = ../../../main.tex


==> 4_multi_task/3_mass/sec/6_related_work.tex <==
%!TEX root = ../../../main.tex


==> 4_multi_task/3_mass/sec/8_reproducibility_statement.tex <==
%!TEX root = ../../../main.tex
All implementation details and hyperparameter settings required to reproduce our results are provided in \cref{sec:mass-approach,sec:mass-experiments} and in \cref{app:additional_details}. Code is provided in \cref{app:additional_details} and will be publicly released along with all the checkpoints and logs. 

==> 4_multi_task/5_merge3/1_Introduction/content.tex <==
%!TEX root = ../../../main.tex

As discussed in \cref{sec:landscape}, merging has significantly broadened access to the field, with ML practitioners producing competitive models on standard consumer GPUs.
%
\begin{figure}[t]
    \centering
    \includegraphics[width=.7\linewidth]{figures/flops_vs_accuracy.pdf}
    \caption[Accuracy vs.\ fitness evaluation FLOPs on Japanese \dataset{GSM8K}]{\textbf{Accuracy on Japanese \dataset{GSM8K} over fitness evaluation FLOPs.} \mergethree is competitive with a model evolved on the full dataset by only using a consumer-grade GPU and $2\%$ of the data (point size reflects data amount).}
    \label{fig:speed_accuracy}
\end{figure}
%
However, although computationally inexpensive, most existing approaches rely on ad-hoc, trial-and-error strategies for selecting merge coefficients, which ultimately limits their downstream performance \citep{ties, yu2024language}.
On the other hand, recent work has shown that evolutionary merging can produce models of unprecedented quality by automating the hyperparameter search for merging coefficients \citep{sakana}.
While this technique can incorporate any standard merging method, such models are absent from public leaderboards, likely due to a mismatch between the high computational demands of evolutionary merging and single-GPU setups typical of merging practitioners.
Indeed, computing the fitness function requires generating and evaluating answers for each dataset element, for each candidate in every evolutionary step. As shown in \cref{fig:speed_accuracy}, the fitness computation alone in the 1,000-trial evolutionary merge from \citet{sakana} requires approximately $4\times10^6$ TFLOPs, with the full algorithm demanding well over a month of continuous computation if run on a single NVIDIA 4090 (\cref{app:add-exp-4090}) with 24 GB of VRAM.
Because it requires repeated and costly forward passes through large language models, fitness evaluation is the primary bottleneck, making evolutionary merging out of reach on consumer hardware and potentially excluding the very users it was meant to empower.

% APPROACH
The framework introduced here, \mergethree{}, addresses this computational barrier by reducing fitness evaluation costs by a factor of $50\times$, making evolutionary merging feasible on a single consumer GPU with competitive results (see \cref{fig:speed_accuracy}). Unlike the approach of \citet{sakana}, \mergethree{} operates with just $0.077 \times 10^6$ TFLOPs, bringing the computation from over a month down to roughly a day on a single NVIDIA 4090.

The approach rests on three steps. First, \textbf{E}xtract: a reduced subset of the fitness evaluation dataset is sampled, significantly alleviating the computational bottleneck of fitness computation (\cref{fig:teaser}). This reduction, however, risks losing accuracy if the subset lacks diversity. To bridge the gap between reduced-dataset evaluations and full-dataset performance, we apply Item Response Theory (IRT) \cite{lord1968statistical}, a well-established statistical framework from psychometrics.
Specifically, the second step, \textbf{E}stimate, uses IRT to infer the latent abilities of the endpoint models, ensuring the merged models accurately reflect their components' strengths. The third step, \textbf{E}volve, optimizes merging coefficients with IRT-based performance estimators designed for model merging, assuming the merged model's ability is a linear combination of those of the endpoints. This integration of merging-specific insights into performance estimation theory maintains high accuracy with drastically reduced datasets.

Experimental results show that \mergethree{} effectively transfers mathematical skills by merging a strong math model with three language-specific models, achieving 10--20\% higher accuracy than standard merging baselines in each language. The framework also evolves a single multilingual model by merging Italian, English, German, and Dutch models, outperforming individually fine-tuned models by up to 19\% on \dataset{ARC} \cite{ARC}. On Japanese \dataset{GSM8K} \cite{gsm8k}, \mergethree{} approximates models evolved on the full dataset while maintaining high efficiency. A modular library for evolutionary merging on consumer GPUs and a suite of state-of-the-art models for several low-resource languages are released alongside this work.



==> 4_multi_task/5_merge3/3_Approach/content.tex <==
%!TEX root = ../../../main.tex
Our method \mergethree speeds up evolutionary model merging by reducing the computational cost of fitness evaluation. It achieves this by shrinking the fitness evaluation dataset and using IRT-based performance estimators to maintain full-dataset accuracy from subset evaluations. \Cref{fig:teaser} shows an overview of the method; the pseudocode for the end-to-end algorithm is given in \cref{alg:merge3}.
%
\begin{algorithm}[ht]
    {\small
    \caption{The full \method{MERGE$^3$} algorithm.} \label{alg:merge3}
    \begin{algorithmic}[1]
    \REQUIRE Dataset $\mathcal{D}$, models $\lbrace M_1, M_2, \ldots, M_n \rbrace$, iterations $T_{\text{iter}}$
    \ENSURE Pareto-optimal merged models
    % \PROCEDURE{MERGE3}{$D, \lbrace M_1, \ldots, M_n \rbrace, T$}
        \STATE $\bar{\mathcal{D}} \gets \Call{RandomSample}{\mathcal{D}, k}$
            \Comment{Sample $k$ items from $\mathcal{D}$}
        \STATE $\lbrace \gamma_1, \ldots,\gamma_n \rbrace \gets \Call{EstimateAbilities}{\{M_1, \ldots, M_n\}, \mathcal{D}}$
        \STATE $P \gets \text{GenerateInitialPopulation}{\{M_1, \ldots, M_n\}}$
        \FOR{$s \gets 1$ to $T_{\text{iter}}$}
            \FORALL{$M \in P$}
                \STATE $\xi \gets \Call{FitXi}{M,\,\lbrace \gamma_1,\dots,\gamma_n \rbrace,\,\bar{\mathcal{D}}}$
                \STATE $\text{preds} \gets \Call{GetPredictions}{M,\,\bar{\mathcal{D}},\,\xi}$
                \STATE $\text{corr} \gets \Call{GetCorrectness}{\text{preds},\,\bar{\mathcal{D}}}$
                \STATE $F(M) \gets \Call{EstimateFitness}{\text{corr},\,\xi}$
            \ENDFOR
            \STATE $P \gets \Call{SelectParents}{P, f}$ 
                \Comment{Select based on fitness}
            \STATE $P \gets \Call{ApplyMutation}{P}$
            \STATE $P \gets \Call{ApplyCrossover}{P}$
                \Comment{Generate offspring}
        \ENDFOR
        \STATE \textbf{return} $\Call{ParetoFront}{P}$
    % \ENDPROCEDURE
    \end{algorithmic}
}
\end{algorithm}

\subsection{Extract \& estimate} \label{sec:extract_and_estimate}
%
Evaluating the fitness function involves generating and assessing answers for each data sample, repeated across all models in the population at every evolutionary step. Given the computational demands of evolutionary algorithms and LLMs, this process is highly intensive. To mitigate this, we reduce the dataset $\mathcal{D}$ to a smaller subset $\bar{\mathcal{D}} \subset \mathcal{D}$ with $|\bar{\mathcal{D}}| \ll |\mathcal{D}|$. After exploring various subsampling strategies, we found uniform random sampling to be as effective as more complex methods (see \cref{app:add-exp:extract-step}) and adopted it for simplicity. 

Reducing the dataset speeds up evaluation but does not guarantee identical results, particularly when the subset is much smaller than the original, as in our setting. To bridge this gap, we build an IRT-based estimator that adjusts for this discrepancy, effectively estimating performance to reflect full-dataset results~\cite{lord1968statistical, tinybenchmarks}.

\label{sec:estimate}

\paragraph{IRT model.}\label{sec:irt}
%
We first define an {estimator} to assess each endpoint model's inherent abilities, derived from the latent variables of a Bayesian model. This ensures that merging preserves individual model strengths. In the Evolve step (\cref{sec:evolve}), the estimated latent abilities are fed to a {\em performance} estimator to compute the final fitness.

To estimate LLM abilities, we build on \citet{tinybenchmarks}, who applied IRT to evaluate LLM performance; however, while they used IRT for benchmarking, we extend it to estimate inherent abilities relevant for model merging, and explicitly use them to guide merging in the Evolve step.

In IRT, latent variables ($\gamma$) represent a model's underlying abilities, while manifest variables ($Y$) indicate response correctness. The framework models the probability of a correct response based on model abilities and item characteristics (e.g., difficulty). IRT defines this probability as:
\begin{equation}
     \mathbb{P}(Y_{im} = 1 \, | \, \gamma_m, a_i, \beta_i) = \frac{1}{1 + \exp(-a_i^\top \gamma_m + \beta_i)} \,
    \label{eq:irt}
\end{equation}
%
Here, ${\gamma_m \in \mathbb{R}^d}$ represents model $m$'s latent abilities, $a_i \in \mathbb{R}^d$ defines the ability dimensions needed to answer example $i$, and $\beta_i$ denotes its difficulty.
%
A model is more likely to answer correctly when its abilities ($\gamma_m$) align with the example's required traits ($a_i$) and less likely when the difficulty ($\beta_i$) is higher.
%
$Y_{im}$ is a binary variable indicating whether model $m$ correctly predicts example $i$ (1 if correct, 0 otherwise).

Crucially, this approach estimates a model's likelihood of answering correctly {\em without directly analyzing the example's content}, relying solely on the estimated IRT parameters ($\gamma_m, a_i, \beta_i$).

\paragraph{Fitting.}\label{sec:fit_irt}
We use variational inference to efficiently estimate both example-specific $(a_i, \beta_i)$ and model-specific ($\gamma_m$) parameters within a hierarchical Bayesian model \citep{lalor2023py}, initialized as detailed in \cref{app:fitting_details}.
Following \citet{tinybenchmarks}, we estimate $a_i$ and $\beta_i$ using correctness data ($Y_{im}$) from publicly available model evaluations, namely the Open LLM leaderboard. 
%
To estimate $\gamma_m$, each endpoint model generates answers for the full evaluation dataset, which are then used to assess correctness ($Y_i$) (see \cref{fig:teaser}). This procedure is repeated for each model $m$, producing the corresponding $\gamma_m$ ($\gamma_1$ and $\gamma_2$ in the figure).

In contrast to prior work, where IRT latent abilities remain hidden variables used only for scoring, we explicitly extract $\gamma_m$ as an {\em ability estimator} that quantifies each model's strengths. Moreover, rather than estimating $\gamma_m$ from a subset, we compute it using the {\em full} evaluation dataset, providing a more comprehensive measure of model ability that directly informs the merging process.

\begin{figure}
    \centering
    \includegraphics[width=0.85\textwidth]{figures/estimation_comparison_main.pdf}
    \caption[Performance estimator error vs.\ sample size]{\textit{Performance Estimators:} Absolute error of various estimators as a function of sample size (lower is better). Our \mpirt{} and \gmpirt{} estimators consistently achieve lower error across various sample sizes and datasets.
     Additional results available in \Cref{fig:estimation_comparison_winogrande_hellaswag}.}
    \label{fig:estimation_comparison}
\end{figure}

\subsection{Evolve: Performance estimator}
\label{sec:evolve}
The \textit{performance estimator}, a key part of the Evolve step, efficiently approximates the fitness function, which measures the merged model's accuracy. Since the fitness function is evaluated once per candidate per evolutionary step, reducing its cost is crucial. Instead of evaluating the full dataset, the estimator predicts performance using only the endpoint models' abilities and the reduced dataset from the previous steps, significantly accelerating the process.

We introduce two novel performance estimators for merging: merged performance Item Response Theory estimator (\mpirt{}) and generalized merged performance Item Response Theory estimator (\gmpirt{}). Since model merging linearly combines weights, we assume that the latent abilities of the merged model (e.g., problem-solving or linguistic capabilities) are also a linear combination of the endpoints' abilities. This assumption mirrors the linear task-vector framework established in \cref{ch:gradient}, where merged parameters are linear combinations of task-specific displacements. It also makes the approach substantially cheaper: we estimate only the interpolation coefficients $\xi$ rather than recomputing the full ability vector $\gamma$ of each merged candidate from scratch (as done in \pirt{} and \gpirt{} \cite{tinybenchmarks}).
%
\begin{assumption}[Linear Combination of Latent Abilities]\label{conj:latent-abilities-linear}
Let \(\{m_0, m_1, \dots, m_n\}\) be endpoint models with latent ability vectors \(\gamma_{i}\). If a new model \(\tilde{m}\) is formed as a linear combination of their parameters, its ability vector \(\gamma_{\tilde{m}}\) can be expressed as:
\begin{align}
    \gamma_{\tilde{m}}
    \;=\;
    \sum_{j=1}^n \xi_j \,\gamma_{j}
    \;=\;
    [\gamma_{1}, \ldots, \gamma_{n}]\,\xi
\end{align}
%
where \(\xi = (\xi_1, \ldots, \xi_n)\) are the interpolation coefficients.
\end{assumption}
%
This assumption allows us to compute the multidimensional IRT model (\cref{eq:irt}) for model merging as a linear combination of the individual models' abilities:
\begin{align}
    p_{i\tilde{m}} 
    &= \mathbb{P}\!\left( Y_{i\tilde{m}} = 1 \;\middle|\; 
    \xi_1 \gamma_{1} + \xi_2 \gamma_{2}, \, 
    a_i, \, \beta_i \right) \nonumber\\
    &= \frac{1}{1 + \exp\!\left(
    -a_i^\top \bigl( \xi_1 \gamma_{1}
    + \xi_2 \gamma_{2} \bigr) 
    + \beta_i \right)}
     \label{eq:prob_model}
\end{align}



%
Since the endpoint models' latent abilities \(\gamma_j\) were pre-estimated over the full dataset \(\mathcal{D}\) in the Estimate step, we only need the subset \(\bar{\mathcal{D}}\) to estimate the interpolation coefficients \(\xi_j\) via MLE.

\paragraph{Performance Estimators.}
To estimate the accuracy of the merged model $\tilde{m}$ using only the reduced dataset $\bar{\mathcal{D}}$ and $p_{i\tilde{m}}$, we define the \emph{merged performance-IRT} (\textsc{mp-IRT}) estimator as:
\begin{align}
    \hat{Z}_{\tilde{m}}^{\mathrm{mp\text{-}IRT}}=
    \frac{\hat{\tau}}{\lvert \bar{\mathcal{D}} \rvert}
    \sum_{i \in \bar{\mathcal{D}}}
    Y_{i\tilde{m}}
    +
    \frac{1 - \hat{\tau}}{\lvert \mathcal{D} \setminus \bar{\mathcal{D}} \rvert}
    \sum_{i \in \mathcal{D} \setminus \bar{\mathcal{D}}} 
    \hat{p}_{i\tilde{m}}
\end{align}
where ${\hat{\tau} = \frac{|\bar{\mathcal{D}}|}{|\mathcal{D}|}}$ downweights smaller subsets that may be noisier. In practice, we are considering the observed correctness for the data points we have access to, while $\hat{p}_{i\tilde{m}}$ predictions are used for the rest of them, enabling accurate performance estimation across all examples despite evaluating only a subset, where $\hat{p}_{i\tilde{m}} = \mathbb{P}\!\left( Y_{i\tilde{m}} = 1 \;\middle|\; \hat{\xi}_1 \hat{\gamma}_{1} + \hat{\xi}_2 \hat{\gamma}_{2}, \, \hat{a}_i, \, \hat{\beta}_i \right)$ is the distribution defined by plugging into \cref{eq:prob_model} the parameters found via MLE. 

Although designed for model merging, \(\hat{Z}_{\tilde{m}}^{\mathrm{mp\text{-}IRT}}\) inherits certain limitations of \(\textsc{p-IRT}\)~\citep{tinybenchmarks}, such as non-uniform weighting and imperfect IRT fits. To mitigate these, we define a \emph{generalized} estimator. Let \(c \in [0,1]\) be a scalar that controls the balance between observed and predicted correctness, and let \(w_i = 1/|\bar{\mathcal{D}}|\) be uniform per-sample weights. The generalized estimator interpolates between \(\hat{Z}_{\tilde{m}}^{\mathrm{mp\text{-}IRT}}\) and the observed correctness on \(\bar{\mathcal{D}}\):
%
\begin{align}\label{gp-irt}
    \hat{Z}_{\tilde{m}}^{\mathrm{gmp\text{-}IRT}}
    \;=\;
    c \sum_{i \,\in\, \bar{\mathcal{D}}} w_i\,\hat{Y}_{i\tilde{m}}
    \;+\;
    (1 - c)\;\hat{Z}_{\tilde{m}}^{\mathrm{mp\text{-}IRT}}
\end{align}
%
We discuss in \cref{app:hyper-search} the optimal choice for \(c\).
Although model merging can sometimes degrade performance due to weight interference, suggesting non-linear ability interactions, our assumption is empirically supported as we are interested only in evolved models that show a positive performance gain. As validated in our experiments (\cref{sec:exp_validation}), our custom estimators, designed around this assumption, outperform standard IRT estimators.


\subsection{Evolve: Evolutionary search}
\label{sec:evolve_evo}  
%
The final step of our algorithm frames model merging as a multi-objective optimization problem.  
Each merging objective \( F(\tilde{m}; D_i) \) represents the performance of the merged model \(\tilde{m}\) on task~\(i\). In practice, we select a multi-objective evolutionary algorithm (e.g., NSGA-II~\citep{nsga-ii}) and a merging strategy (e.g., TIES~\citep{ties}), aiming to optimize the corresponding {Pareto front}, formally defined as:  
\[
P_{\overline{F}_D}(\Theta)
\;=\;
\bigl\{
\theta_i \,\in\, \Theta 
:\; \nexists\,\theta_j \,\in\, \Theta
\;\text{s.t.}\;\theta_j \succ \theta_i
\bigr\}
\]  
where \(\succ\) denotes \emph{Pareto-dominance}. A model \(m\) Pareto-dominates \(m'\) if:  
\begin{align*}
\forall \, F \,\in\, \overline{F}_D:\; 
F(m; D) &\leq F(m'; D)\\
&\quad\text{and}\\
\exists \, F \,\in\, \overline{F}_D:\; 
F(m; D) &< F(m'; D)
\end{align*}  
This means \(m\) is strictly better in at least one metric and no worse in all others. Models on the Pareto front are thus not dominated by any other model.

In our setting, to reduce computational costs, we approximate optimization using \(\overline{F}_{\bar{\mathcal{D}}}\) instead of \(\overline{F}_{\mathcal{D}}\), where \(\bar{\mathcal{D}} \subset \mathcal{D}\) is obtained by the \textit{extraction} step. Performance on \(\bar{\mathcal{D}}\) is then estimated using the {performance estimator}.  




==> 4_multi_task/5_merge3/4_Experiments/content.tex <==
%!TEX root = ../../../main.tex
\begin{figure}
    \centering
    \includegraphics[width=.8\linewidth]{figures/latent_abilities_tasks_main.pdf}
    \caption[Ability estimator cosine similarity comparison]{\textit{Ability Estimator:} Cosine similarity between estimated and true abilities for different tasks (higher is better). Our estimated abilities $\gamma^{\{\mathrm{mp},\mathrm{gmp}\}-{\mathrm{IRT}}}$ better approximate true abilities.}
    \label{fig:ability-estimator-comparison}
\end{figure}

\begin{figure}
    \centering
    \begin{subfigure}{0.32\linewidth}
        \includegraphics[width=\linewidth]{figures/cross-Romanian.pdf}
        \caption{To Romanian.}
        \label{fig:cross-ro}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.32\linewidth}
        \includegraphics[width=\linewidth]{figures/cross-German.pdf}
        \caption{To German.}
        \label{fig:cross-de}
    \end{subfigure}
    \begin{subfigure}{0.32\linewidth}
        \includegraphics[width=\linewidth]{figures/cross-Dutch.pdf}
        \caption{To Dutch.}
        \label{fig:cross-nl}
    \end{subfigure}
    \caption[Cross-lingual math skill transfer via model merging]{\textit{Cross-lingual skill transfer}: merging math models (dark blue) with language-specific models (red) effectively transfers mathematical skills across languages (green - our method) compared to baselines (white). Accuracy on \dataset{GSM8K} for each target language.
        %, with white indicating baseline merging approaches.
    }
    \label{fig:cross-transfer}
\end{figure}
%
In this section, we evaluate \mergethree, demonstrating its effectiveness in
evolutionary model merging on consumer-grade GPUs. We first validate the
proposed ability and performance estimators, assessing their accuracy in
approximating full-dataset evaluations. Next, we examine cross-lingual
transfer, where \mergethree enables efficient merging of multilingual models,
improving mathematical reasoning across languages. Thereafter, we evaluate its
ability to synthesize multilingual models, surpassing individual fine-tuned
baselines while remaining computationally efficient. Finally, we analyze the
performance of \mergethree on different GPUs. All merging experiments were
performed with our library \textit{Mergenetic}~\citep{minut2025mergenetic} (see Appendix
\ref{app:mergenetic}) on an RTX 4090 GPU featuring 24 GB of VRAM, while
employing a batch size of 8, $4$-bit quantization, and models comprising
$\approx 7$ billion parameters (see Appendix \ref{app:add-details}).

\subsection{Validating estimators}
In this section, we empirically validate our merged-performance estimators by
comparing them against standard \pirt{} and \gpirt{} estimators
\cite{tinybenchmarks} across five benchmark datasets: \dataset{GSM8K}
\cite{gsm8k}, \dataset{Winogrande} \cite{sakaguchi2021winogrande},
\dataset{TruthfulQA} \cite{lin2021truthfulqa}, \dataset{Hellaswag}
\cite{zellers2019hellaswag}, and \dataset{ARC} \cite{ARC}. Additional results are provided in \cref{app:add-exp}.

\paragraph{Ability Estimators.}
\label{sec:exp_validation}
%
To validate our ability estimators we compare their inferred latent ability
vectors to the reference ``ground-truth'' vectors \(\Gamma\). Specifically, we
measure the cosine similarity and the Euclidean distance from the ground-truth
\(\Gamma\) both for \(\gamma^{{\{\mathrm{mp,gmp}\}-\mathrm{IRT}}}\), estimated
with our merged-performance IRT approaches, and
\(\gamma^{\{\mathrm{p,gp}\}-\mathrm{IRT}}\), estimated with the \pirt{} and
\gpirt{} estimators \citep{tinybenchmarks}. Here, \(\Gamma_{m}\) is computed by
fitting the IRT model (as in \cref{sec:irt}) to each merged model \(m\) using
its entire set of responses on the full dataset \(D\). Incorporating all
available data, \(\Gamma_{m}\) serves as our best proxy for the model's true
ability. Conversely, both \(\gamma_m^{{\{\mathrm{mp,gmp}\}-\mathrm{IRT}}}\) and
\(\gamma_m^{\{\mathrm{p,gp}\}-\mathrm{IRT}}\) are estimated using only a
smaller subset \(\bar{D} \subset D\) of size \(n\).
\Cref{fig:ability-estimator-comparison} shows the results of this comparison
for $n=10$ and $n=20$, while the results for $n=15, 30, 50, 100$ are reported
in \Cref{app:estimation-step} along with the same experiment over different
languages. Across all five benchmark tasks, our proposed ability estimator
\(\gamma_m^{{\{\mathrm{mp,gmp}\}-\mathrm{IRT}}}\) consistently yields ability
vectors with higher cosine similarity to \(\Gamma\) than
\(\gamma_m^{\{\mathrm{p,gp}\}-\mathrm{IRT}}\). This trend is evident across
both subset sizes, highlighting the robustness of our approach even with
limited data. The superior performance of
\(\gamma_m^{{\{\mathrm{mp,gmp}\}-\mathrm{IRT}}}\) empirically validates
\Cref{conj:latent-abilities-linear}, confirming that an IRT-based ability
estimator designed around this assumption provides more accurate ability
estimates than a general-purpose alternative.

\paragraph{Performance Estimators.} \label{par:pe}
%
To assess the accuracy of our proposed performance estimators, we measure their
absolute estimation error across different sample sizes. Specifically, we
evaluate the performance estimates of six merged models using random sampling,
\pirt{}, \gpirt{} \cite{tinybenchmarks}, \mpirt{}, and \gmpirt{} across various
subset sizes. The resulting absolute errors shown in
\cref{fig:estimation_comparison} are reported for \dataset{ARC},
\dataset{GSM8K}, \dataset{TruthfulQA}, and an aggregate average across all five
benchmarks.

As shown in the figure, our proposed estimators, \mpirt{} and \gmpirt{},
consistently achieve lower absolute error compared to \gpirt{} and \pirt{}.
While all IRT-based methods outperform random sampling, the incorporation of
merged-performance IRT significantly enhances estimation accuracy. Notably,
both \mpirt{} and \gmpirt{} maintain low empirical error and reduced variance
even when operating with very small subsets (\(|\bar{D}| \approx 1.5\%\) of the
full dataset). This highlights the robustness of our approach in low-data
regimes.

Since lower empirical error often correlates with reduced \emph{expected} error
(as formalized in Section~\ref{sec:theory}), we adopt \mpirt{} and \gmpirt{} as
our primary estimators for evolving merged language models in subsequent
experiments.

\begin{figure}
    \centering
    \includegraphics[width=.7\linewidth]{figures/comparison-Sakana.pdf}
    \caption{Accuracy of merged models for Japanese \dataset{GSM8K}.}
    \label{fig:evolve-comparison-sakana}
\end{figure}

% Math transfer to DE, RO, NL, Jap
\subsection{Cross-lingual transfer of mathematical skills}
\label{sec:cross-lingual}
To assess the transfer of mathematical reasoning from English to other languages, we merge an English math-specialized model with a \model{Mistral-7B} \cite{mistral} fine-tuned on each target language, then evaluate on the corresponding \dataset{GSM8K} translations \citep{gsm8k}. Appendix \ref{app:add-details-evo} provides details on the specific models used for merging. Following \citet{sakana}, we label an answer correct only if it is both accurate and written in the target language. We benchmark our approach against three commonly used merging baselines: \method{Task Arithmetic} \citep{task-vectors}, \method{TIES} \citep{ties}, and \method{DARE} \citep{yu2024language}. Following standard practice in the merging community, we apply either \method{TIES} and \method{DARE} jointly, or \method{SLERP} \cite{10.1145/325165.325242}.

As shown in \cref{fig:cross-transfer}, merging a language-specific fine-tuned model
with a math-specialized model consistently surpasses both endpoint models by
10--20\% in accuracy on the translated \dataset{GSM8K}. In contrast, standard
baselines often yield sub-optimal merges, performing worse than the endpoints
themselves. This highlights the importance of optimized merging coefficients
and motivates our evolutionary framework.

% To rule out the possibility that gains arise merely from exploiting a small, in-distribution dataset---rather than true cross-lingual transfer---we also merge the same Italian fine-tuning with itself; the results, available in the appendix \ref{sec:self-merging}, shows no improvement, reinforcing that our observed gains stem from genuine knowledge transfer.

Next, we evaluate our method for transferring math skills from English to
Japanese and compare it to \method{EvoMerge} \citep{sakana}, which serves as an
upper bound by computing fitness on the full dataset. As illustrated in \cref{fig:evolve-comparison-sakana}, our approach confirms the significant gains
seen for the other languages, greatly surpassing both the performance of the
endpoint models and that of the merging baselines. While the accuracy is lower
than that of the model obtained by computing the fitness on the full dataset as
done by \citet{sakana}, \cref{fig:speed_accuracy} shows that our
approximation yields a method that is $50\times$ more efficient, effectively
making evolutionary merging feasible on a single NVIDIA 4090 GPU (see \cref{tab:multi_gpu_timing} for timings across different hardware).

\subsection{Ablation study: self-merging}
\label{sec:self-merging}
%
\begin{wrapfigure}[14]{r}{0.45\textwidth}
    \vspace{-0.5cm}
    \centering
    \includegraphics[width=\linewidth]{figures/self-merge.pdf}
    \caption[Self-merging ablation on Italian \dataset{GSM8k}]{Accuracy of the base model (Mistral-7B), the Italian Endpoint (\texttt{IT}), Self-Merge and \mergethree models on the Italian-translated version of \dataset{GSM8k}.}
    \label{fig:self-merge}
\end{wrapfigure}
In this section, we present an ablation study to test whether the observed improvements in the merged models arise from genuine cross-lingual knowledge transfer or merely from fitting to the prompt template. To structure this analysis, we formalize our inquiry through two hypotheses:

\textit{Null Hypothesis ($H_0$).} The improvements seen in the merged models are due to the model fitting itself on the prompt template, rather than any cross-lingual knowledge exchange.

\textit{Alternative Hypothesis ($H_1$).} The improvements arise from actual cross-lingual knowledge transfer and are not merely the result of fitting the prompt template.

To evaluate these hypotheses, we propose a \emph{self-merging} procedure.
Concretely, we take the linguistic model and merge it with \emph{itself} using
the standard \mergethree methodology outlined in \cref{alg:merge3}. Under $H_0$,
if the improvements are solely due to the prompt template, merging the model
with itself should lead to performance gains (i.e., the merged model would
still ``fit'' the template). Conversely, under $H_1$, if cross-lingual
knowledge transfer is responsible for the enhanced performance, self-merging
should \emph{not} yield improvements. In fact, additional noise could even
degrade performance relative to the baseline.

We conducted this self-merging experiment on the Italian model using the
\dataset{GSM8K} dataset. The results, shown in \cref{fig:self-merge}, reveal
that performance actually \emph{decreases} when the model is merged with
itself. This observation strongly supports the alternative hypothesis ($H_1$):
the performance gains in cross-lingual merges indeed stem from genuine
knowledge transfer, rather than mere adaptation to a prompt template.
%
%
\subsection{Evolving a multilingual model}
\label{sec:multi-lingual}

\begin{table}
    \centering
    \begin{tabular}{ccccccccc}
        \\
        \toprule
        \multirow{2}{*}{Model} & \multicolumn{8}{c}{\textbf{Accuracy} ($\uparrow$)}                                                                                                                                                            \\
        \cmidrule{2-9}
                               & \multicolumn{2}{c}{Italian}                        & \multicolumn{2}{c}{English} & \multicolumn{2}{c}{German} & \multicolumn{2}{c}{Dutch}                                                                     \\
        \midrule
        Finetuned              & 0.61                                               & --                          & 0.75                       & --                        & 0.61          & --              & 0.50          & --              \\
        \mergethree             & \textbf{0.69}                                      & \improvUP{8\%}              & \textbf{0.79}              & \improvUP{4\%}            & \textbf{0.72} & \improvUP{11\%} & \textbf{0.69} & \improvUP{19\%} \\
        \bottomrule
    \end{tabular}
    \caption[Evolved multilingual model accuracy on \dataset{ARC}]{Evolving a multilingual model. For each language, we report the accuracy on the corresponding translated \dataset{ARC} of both the language-specific model and the evolved multilingual model.}
    \label{tab:multilingual}
\end{table}
We next combine individually fine-tuned models for \{\texttt{IT, EN, DE, NL}\} into a single multilingual model. Appendix \ref{app:add-details-evo} provides details on the specific models used for each language. As shown in \cref{tab:multilingual}, the resulting merged model surpasses each language-specific variant by up to 19\% in accuracy on the \dataset{ARC} dataset \cite{ARC}. Even more notably, it outperforms all its constituent endpoints, demonstrating a clear positive transfer of knowledge across languages.
Notably, the largest improvement occurs for Dutch (from 50\% to 69\%), suggesting that merging particularly benefits languages where baseline performance is lower. Even English, which starts from the highest baseline, gains by 4\%, indicating that positive transfer is not limited to stronger endpoints. The fact that the merged model outperforms all individual fine-tunings (rather than landing between them) points to a genuine cross-lingual synergy. These conclusions are further strengthened by the self-merging ablation in \cref{sec:self-merging}.

==> 4_multi_task/5_merge3/Z_Misc/content.tex <==
%!TEX root = ../../../main.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% INTRO TO TINY BENCHMARKS AND APPROXIMATION CONJECTURE

Emergent abilities in LLMs have a steeper learning curve than the simple loss functions they are trained on. This justifies the term "emergent" as models suddenly begin to perform well on certain tasks during the training process. A steeper learning curve in the parameter space means that performance differences are more pronounced, allowing us to use fewer data points to approximate the performance order of models. Consequently, it becomes less computationally expensive to evaluate whether the performance of the merged model has degraded or improved compared to the original model on a given task $t_j$ entangled in a language $L_i$, such as math word problems or common sense reasoning.
\begin{conjecture}\label{conj:approx}
    The order between two language models $\theta_{a}$ and $\theta_{b}$ with regard to a metric $M$ measuring an emergent ability $t$ over a labeled dataset $X_{t}=\{(x_i,y_i)\}_{i=0}^n$ can be correctly approximated by their performance on a subset $\hat{X_t} \subset X_t$.
\end{conjecture}
While this order remains an approximation, it can still be sufficient for an evolutionary algorithm to converge towards an optimum. 
\texttt{tinyBenchmarks} \citep{tinybenchmarks} allows to estimate the performance of a LLM $l$ on the dataset $I_j$ by leveraging its predictions on the subset $\hat{I_j}$. Nevertheless, in the field of evolutionary model merging, we can estimate the performance of $l_m$ by leveraging the evaluation of the merged model $l_m$ on $\hat{I_j}$, but also relying on the full evaluations of the component models $l_1,...,l_k$ over the dataset $I_j$.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% ON THE BENEFITS OF mp-IRT vs p-IRT in model merging 

Normally, we would have estimated $\hat{\gamma}_{\tilde{m}} \approx \gamma_{\tilde{m}}$ on $\hat{D}$ by finding the MLE estimator of  $\gamma_{\tilde{m}}$ by maximizing the likelihood of $Y_{(\hat{D},\tilde{m})}$. Nevertheless, this faces the following challenges: 
%
\begin{enumerate*}[label=(\roman*)]
  \item it does not use the available data about $m_1$ and $m_2$, namely $Y_{(D,m_1)}$ and $Y_{(D,m_2)}$;
  \item when merging LLMs, the ability required for solving a simple task/item $i$ are several, and therefore the number of abilities that must be modeled to get an adequate $|\gamma|$ may grow significantly. This may require more data to get a good estimation of the latent ability $\gamma$ of the model.
\end{enumerate*}


\subsection{Task Vectors vs Language Vectors}
Inspired by task vectors~\citep{task-vectors, crossmerge}, we define a language vector as:
%
\begin{equation}
    \tau_{L_t} = \theta_{(L_t,L_s)} - \theta_{L_s}
\end{equation}
%
where $\theta_{L_s}$ is the language model pre-trained in the source language $L_s$, and $\theta_{(L_t,L_s)}$ is the model obtained after fine-tuning $\theta_{L_s}$ on unlabeled data in the target language $L_t$. Although the definition of a language vector closely resembles that of a task vector, they tend to differ significantly in practice. Task vectors are typically derived from training models on supervised tasks that are quite different from one another (e.g., MNIST and EuroSAT~\citep{task-vectors}). In contrast, language vectors are obtained from fine-tuning models on unlabeled generic datasets, which theoretically differ only in language. As a result, language vectors tend to be more similar to each other~\cite{notrain}, resulting in a much higher cosine similarity than task vectors~\citep{notrain}. This increased similarity may complicate the process of obtaining good merged models, as \citet{task-vectors} speculate that the orthogonality of task vectors helps prevent weight interference, which is crucial for successful model merging.


\subsection{The Language-Task Analogy Challenge}

% Task vectors also allow computing analogies, generalizing a model $\theta_{(t,a)}$ trained on a specific task $t$ (e.g, NER) in domain $a$ (e.g., finance) to a new domain $b$ (e.g., law). This is achieved by combining the supervised fine-tuning of $\theta_{(t,a)}$ on domain $a$ and task $t$ with two unsupervised fine-tunings of $\theta_0$ on domains $a$ and $b$, namely $\theta_{a}$ and $\theta_{b}$. The analogy function is given by:
% \[
%     F_{\text{analogy}}(\theta_0, \theta_a, \theta_b, \theta_{(t,a)}) = (\tau_{b} - \tau_{a}) + \tau_{(t,a)} + \theta_0 \approx \theta_{(t,b)}.
% \]

Previous approaches \cite{crossmerge} have deployed on task analogies \cite{task-vectors} to achieve cross-language transfer. This relies on the intuitive relationship: "task $\text{t}_{(j,l_1)}$ is to language $l_1$ as task $\text{t}_{(j,l_2)}$ is to $l_2$". However, in most cases, merging multilingual models through language-task analogies is unfeasible for decoder-only architectures. The task one aims to transfer across languages is often entangled with the source language of the training dataset, reducing the language-task analogy to mere addition.

\begin{theorem}\label{thm:impossibility-task-analogies}
    Given a model $\theta_{L_i} \in \mathbb{R}^{d}$ proficient in a language $L_i$, a model $\theta_{(f_k, L_i)} \in \mathbb{R}^{d}$ proficient in the task $f_k$ entangled with $L_i$, and a model $\theta_{L_j} \in \mathbb{R}^{d}$ proficient in language $L_j$, if $L_{source} = L_{i}$, then:
    $$
        F_{analogy}(\theta_{L_{source}}, \theta_{L_i}, \theta_{L_j}, \theta_{(f_k, L_i)}) = F_{addition}(\theta_{L_{source}}, \theta_{(f_k, L_i)}, \theta_{L_j})
    $$
\end{theorem}

where $F_{analogy} : \mathbb{R}^{d \times 4} \to \mathbb{R}^{d}$ maps four models to an analogy model, and $F_{addition} : \mathbb{R}^{d \times 3} \to \mathbb{R}^{d}$ maps three models to an arithmetic model. $L_{source}$ is the language of the pre-trained model $\theta_{L_{source}}$. 
Due to the lack of supervised datasets for low-resource languages, most tasks one may want to transfer to a language model in $L_{target}$ are entangled with $L_{source}$, which is often English. This makes language-task analogies an impossible solution for generalizing capabilities from English to low-resource languages in the context of large models such as Mistral \cite{mistral}.

To sum up, creating effective multilingual models presents significant challenges which can be addressed with model merging. However, when applying model merging to the domain of multilinguality and cross-lingual transfer, additional obstacles must be overcome to develop effective Multilingual Language Models (MLLMs):

\begin{itemize}
    \item The trial-and-error approach of model merging \cite{surveydmf} is less effective due to the higher difficulty posed by language vectors compared to task vectors, primarily because of their high cosine similarity \cite{crossmerge}.
    \item When working with popular English autoregressive monolingual LLMs, the abilities intended for transfer to low-resource languages through fine-tuning are often derived from tasks entangled with English. This makes it impossible to use task-language analogies, as they reduce to task-language arithmetic (Theorem 1).
\end{itemize}

Model merging, while promising, requires solving these additional challenges to achieve effective cross-lingual transfer and the development of robust MLLMs.





% CROSS-LINGUAL TRANSFER
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Our first set of experiments focused on cross-lingual transfer utilizing the Mistral-7B architecture. The results clearly indicate that the EMULI merging method can successfully transfer mathematical capabilities from an English fine-tuned model to an Italian fine-tuned model. This was evidenced by the merged model's ability to solve Italian math problems, achieving performance levels that surpassed the individual models. Moreover, the subsequent merging with a code-generating model demonstrated that the cross-lingual capability extended beyond a single task, addressing RQ2 effectively. The merged model performed well in both math and coding tasks, indicating that the transfer of capabilities was not confined to the initial task but could generalize to other domains.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% MULTI-LINGUAL
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

By merging models fine-tuned in different languages (Portuguese, Turkish, and English; Italian, Dutch, and English), we were able to produce multilingual models that preserved the performance of the original monolingual models while also enabling cross-lingual transfer. The use of NSGA-II for multi-objective optimization proved beneficial. The merged models not only maintained the original linguistic capabilities but, in some cases, even enhanced them. This improvement was particularly notable in the Portuguese, Italian, and Dutch components, showcasing the potential of cross-lingual transfer to bolster model performance in multilingual settings.

% SO VS MO
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Multi-objective optimization consistently outperformed single-objective optimization in most scenarios, except for the Portuguese-Turkish-English experiment. This suggests that as the complexity of the optimization task increases (with more languages and objectives), the benefits of multi-objective optimization become more pronounced.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The results presented highlight the efficacy of our proposed approach for both cross-lingual transfer and the generation of multilingual models through evolutionary model merging. The experiments demonstrate the potential of using evolutionary algorithms to create merged models that retain and enhance the capabilities of the original monolingual fine-tunes, facilitating effective cross-lingual transfer and multilingual model generation.


The extension of our approach to include additional languages (German, Spanish, and Romanian) demonstrated the scalability of our method. The results showed that our approach could generate models proficient in multiple languages, with most of the languages (except Romanian and Italian) greatly benefiting from the cross-lingual transfer of capabilities. However, it is worth noting that we could only evaluate 1 model of the Pareto front, and by testing additional merged models we may observe an improvement even for Romanian and Italian.


The comparison with baseline models created using task arithmetic with uniform weights underscored the necessity of evolutionary optimization. The baseline models failed to transfer capabilities effectively, resulting in significantly lower performance. This highlights the importance of a structured optimization framework when dealing with language vectors, as the complexity of merging multiple language models demands a more sophisticated approach than simple averaging.

Overall, the results affirm the effectiveness of our evolutionary model merging approach for both cross-lingual transfer and multilingual model generation. The EMULI merging method provides a robust framework for creating high-performing multilingual models that retain and enhance the capabilities of their monolingual counterparts. 

==> 4_multi_task/5_merge3/preamble.tex <==
%!TEX root = ../../main.tex
\usepackage{times}
\usepackage{graphicx}
\usepackage{booktabs}
\usepackage{xcolor}
\usepackage{amsmath, amsthm, amssymb, amsfonts}
\usepackage{thmtools}
\usepackage{graphicx}
\usepackage{setspace}
%\usepackage{geometry}
\usepackage{float}
\usepackage{hyperref}
\usepackage[utf8]{inputenc}
\usepackage[english]{babel}
\usepackage{framed}
\usepackage{cleveref}
\usepackage[inline]{enumitem}
\usepackage{hyperref}
\usepackage{url}
\usepackage{wrapfig}
\usepackage{subcaption}
\usepackage{comment}
\usepackage{multirow}


\newcommand{\HRule}[1]{\rule{\linewidth}{#1}}

\newtheorem{theorem}{Theorem}
\newtheorem{conjecture}{Conjecture} 
\newtheorem{assumption}{Assumption}
\declaretheoremstyle[
    headfont=\bfseries, 
    bodyfont=\normalfont, 
    spaceabove=6pt, 
    spacebelow=6pt
]{defsty}
\declaretheorem[style=defsty,numberlike=theorem]{definition}

\declaretheoremstyle[
    headfont=\bfseries, 
    bodyfont=\normalfont, 
    spaceabove=6pt, 
    spacebelow=6pt
]{defsty}
\declaretheorem[style=defsty,numberlike=theorem]{challenge}

\declaretheoremstyle[name=Proposition,]{prosty}
\declaretheorem[style=prosty,numberlike=theorem]{proposition}

\declaretheoremstyle[name=conjecture,]{prcpsty}

\input{math_commands.tex}


% \title{\begin{center}$E^3$-Merging:\\ \textbf{E}xtract Data, \textbf{E}stimate Abilities, \textbf{E}volve LLMs\end{center}}
\icmltitlerunning{MERG$E^3$: Fast Evolutionary Merging via \\ Data Extraction and Ability Estimation}

% The \author macro works with any number of authors. There are two commands
% used to separate the names and addresses of multiple authors: \And and \AND.
%
% Using \And between authors leaves it to \LaTeX{} to determine where to break
% the lines. Using \AND forces a linebreak at that point. So, if \LaTeX{}
% puts 3 of 4 authors names on the first line, and the last on the second
% line, try using \AND instead of \And before the third author name.

%\newcommand{\fix}{\marginpar{FIX}}
%\newcommand{\new}{\marginpar{NEW}}
\newcommand{\mergethree}[0]{MERGE$^3$}
\newcommand{\approach}[0]{MERGE$^3$~}
\newcommand{\mergethreebf}[0]{$\mathbf{\text{MERGE}^3}$}
\newcommand{\model}[1]{\texttt{#1}}
\newcommand{\dataset}[1]{\texttt{#1}}
\newcommand{\method}[1]{\texttt{#1}}
\newcommand{\lang}[1]{\texttt{#1}}


\newcommand{\improv}[1]{\scriptsize{\color{PineGreen}($\downarrow$#1)}}
\newcommand{\improvUP}[1]{\color{PineGreen}($\uparrow$#1)}
\newcommand{\improvDOWN}[1]{\scriptsize{\color{PineGreen}($\downarrow$#1)}}
\newcommand{\degrad}[1]{\scriptsize{\color{BrickRed}($\downarrow$#1)}}
\newcommand{\degradDOWN}[1]{\scriptsize{\color{BrickRed}($\downarrow$#1)}}
\newcommand{\degradUP}[1]{\scriptsize{\color{BrickRed}($\uparrow$#1)}}
\newcommand{\nochange}[1]{\scriptsize{\color{black}(-#1)}}






==> pages/quotepage.tex <==
%!TEX root = ../main.tex

\vspace*{0.2\textheight}

\noindent \emph{``No tears, it's a waste of good suffering.''}\bigbreak

\hfill Hellraiser
